Testing Large-Scale Structure Measurements Against Fisher Matrix Predictions

We compare Baryonic Acoustic Oscillation (BAO) and Redshift Space Distortion (RSD) measurements from recent galaxy surveys with their Fisher matrix based predictions. Measurements of the position of the BAO signal lead to constraints on the comoving angular diameter distance $D_{M}$ and the Hubble distance $D_{H}$ that agree well with their Fisher matrix based expectations. However, RSD-based measurements of the growth rate $f \sigma_{8}$ do not agree with the predictions made before the surveys were undertaken, even when repeating those predictions using the actual survey parameters. We show that this is due to a combination of effects including degeneracies with the geometric parameters $D_{M}$ and $D_{H}$, and optimistic assumptions about the scale to which the linear signal can be extracted. We show that measurements using current data and large-scale modelling techniques extract an equivalent amount of signal to that in the linear regime for $k < 0.08 \,h\,{\rm Mpc}^{-1}$, remarkably independent of the sample properties and redshifts covered.

==> 2nd_V_Testing_Large-Scale Structure_Measurements_Against_Fisher_Matrix_Predictions/table1.tex <==

\begin{table}[t]
\caption{\label{tab:summary} A list of fiducial cosmologies used for each survey in the Fisher analysis.\\}
\centering
 \begin{tabular}{||c | c c c c c c ||} 
 \hline
 Survey & $\Omega_m$	& $\Omega_b$ & $h$ & $\sigma_8$ & $n_s$ & $\Omega_{\nu}$  \\ [0.5ex] 
 \hline\hline

 6dFGS &0.3 &0.0478 &0.70 &0.82 &0.96 &  0 \\
 \hline
 MGS	&0.31	&0.048	&0.67	&0.83	&0.96	&0	 	\\
 \hline
 BOSS (DR12)	&0.31	&0.04814	&0.676	&0.8	&0.97	&0	 \\
 \hline
 BOSS (DR9-11)	&0.274	&0.0457	&0.70	&0.8	&0.95	&0	 \\
 \hline
 eBOSS	&0.31	&0.04814	&0.676	&0.8	&0.97	&0.0014	 \\
 \hline
 WiggleZ &0.27 &0.04483 &0.71 &0.8 &0.963 &0  \\ 
 \hline
\end{tabular}
\end{table}

==> 2nd_V_Testing_Large-Scale Structure_Measurements_Against_Fisher_Matrix_Predictions/table2.tex <==

\begin{table}[t]
\caption{\label{tab:results} The Fisher forecast (shortened as F.) errors for $D_M$, $D_H$, $D_V$, and $f\sigma_8$ compared to the errors from the BAO and RSD measurements (shortened as O.). The RSD rows show $f\sigma_8$ errors from observations with and without marginalisation over the dilation parameters (Mg. for marginalized and Fx. for fixed).
%\Alex{Can we add an additional row for kmax in the data?}
For 6dFGS, the sample used for RSD has slightly different
$b_{\rm eff}$ and $z_{\rm eff}$ from the sample used for BAO;
in the Fisher forecast we use $b_{\rm eff}$ and $z_{\rm eff}$ from ref.~\cite{carter_low_2018} for both, for consistency.
The BOSS analysis have used 4 different RSD models that were briefly described in the text. The eBOSS $\rm LRG^{+}$ sample reported in this table is the combined eBOSS LRG sample covering $4,242 \rm \ deg^2$ with the BOSS DR12 sample at high redshift ($0.6<z<1.0$), covering $9,494 \rm \ deg^2$.
We also display the $k_{\rm max}$ of the observations (converted from configuration to Fourier space if applicable);
the fiducial Fisher $k_{\rm max}$; the $k_{\rm max}$ at which the Fisher RSD constraints
match the observations; the RSD model
used; whether the fit was performed
in configuration ($s$) or Fourier ($k$)
space; and the references for the RSD and BAO papers.
\\ }
\begin{tabular}{||c||c|c|c c|c c c|c c c||}
\hline\hline
  & 6dFGS
  & MGS 
  & \multicolumn{2}{c|}{BOSS} 
  & \multicolumn{3}{c|}{eBOSS} & \multicolumn{3}{c||}{WiggleZ}\\
  &
  & 
  & Near  &  Mid
  & $\rm LRG^{+}$ & ELG & QSO 
  & Near&	Mid&	Far
  \\
\hline
$z_{\rm eff}$ 
& 0.097 & 0.15 & 0.38 & 0.51 & 0.698 & 0.845 & 1.48 & 0.44 & 0.600 & 0.73 \\

$A_{\rm eff}(deg^2)$  
& 17000 & 6813 & 9329 & 9329 & 4242 & 727 & 9494 & 816 & 816 & 816\\

$V_{eff}(Gpc^3)$ & 0.134& 0.282 & 3.401 & 4.082 & 2.652 & 0.522 & 0.525 & 0.288 & 0.364 & 0.223\\

$b_{\rm eff}$
&1.65&1.5&2.03&2.13&2.2&1.52&2.33&1.0&1.1&1.2\\
%for Quasars: table 10 in Neveux et al., (b1NGC * N_NGC + b1SGC * N_NGC) / Ntot
%WiggleZ in https://arxiv.org/pdf/1401.0358.pdf after eq. 3 they. state this is the bias they assumed.

\hline\hline
\multicolumn{11}{c}{Fractional errors from the BAO analysis (in percent)}\\
\hline\hline

$D_M$ (O.)&
&  &  1.5&	1.4&    1.6&       4.3& 	2.5&		 &     &  \\

$D_M$ (F.)&
8.0&  6.4&	1.5&	1.3&	1.7&	3.6&	3.4&	6.9&	6.0&	7.5\\	
\hline

$D_H$ (O.)&
& 	 &  2.7&	2.3&	2.5&	  9.0&	4.0&		 &		 &       \\
$D_H$ (F.)&
16.1&  13.8&	3.1&	2.8&	3.2&	6.3&	5.0&	11.3&	9.5&	11.4\\
\hline

$D_V$ (O.)&
4.6&    3.8&    1.0&	0.9&    1.6&    2.7&  1.5&	4.8&	4.5&	3.4	\\
$D_V$ (F.)&
5.8&    4.9&    1.1&	1.0&	1.2&	2.5&	3.0&	4.6&	3.9&	4.9	\\

\hline\hline

BAO ref. 
& \cite{carter_low_2018}
& \cite{ross_clustering_2015}
&\cite{alam_clustering_2017}
&\cite{alam_clustering_2017}
&\cite{bautista_completed_2020}
&\cite{de_mattia_completed_2020}
&\cite{neveux_completed_2020}
&\cite{kazin_wigglez_2014}
&\cite{kazin_wigglez_2014}
&\cite{kazin_wigglez_2014}\\

\hline\hline
\multicolumn{11}{c}{Fractional errors from the RSD analysis (in percent)}\\
\hline\hline

$f \sigma_8$(O.Mg.)&
&  40.5&	7.8&	7.6&	7.9&
23.6&	9.3&	19.4&	16.1&	16.4	\\
$f \sigma_8$(O.Fx.)&
13.0&  31.8&	7.0&	6.4&	7.6&	 15.2&  6.3&	13.2&	10.9&	8.7	    \\
$f \sigma_8$(F.Fx.)&
19.5&   15.0&	3.7&	3.2&	3.1&	4.4&	4.0&	7.0&	5.6&	6.6\\

\hline\hline
\multicolumn{11}{c}{$k_{max}$ for the RSD modeling}\\
\hline\hline

$k_{\rm max}$(O.)&
0.23&  0.14&  0.17&  0.17&  0.16&
0.16&	0.24&	0.2&	0.2&	0.2\\

$k_{\rm max}$(Fid.\, F.)&
0.11&  0.11&	0.12&	0.13&	0.14&	0.15&	0.20&	0.12&	0.13&	0.14	\\
$k_{\rm max}$(Match)&
0.16&   0.06&	0.08&	0.08&	0.07&	0.06&	0.08&	0.07&	0.07&	0.11 \\	


\hline
RSD Model&
Sc.  &  CLPT&  
\multicolumn{2}{c|}{4 Models}& 
\multicolumn{3}{c|}{TNS\&CLPT+GS}&
\multicolumn{3}{c||}{J+11}
%From section 3.2 of this paper: https://academic.oup.com/mnras/article/418/3/1725/1062307?login=true

%0.15 in BOSS comes from Beutler et al. 2017b paper monopole and quadrupole.
\\


 RSD space&
 $s$ &
 $s$ &
 $k$/$s$ &
 $k$/$s$ &
 $s$ &
 $k$/$s$ &
 $k$/$s$ &
 $k$ &
 $k$ &
 $k$ \\


RSD ref. 
& \cite{beutler_6df_2012}
& \cite{howlett_clustering_2015}
&\cite{alam_clustering_2017}
& \cite{alam_clustering_2017}
&\cite{bautista_completed_2020}
&\cite{de_mattia_completed_2020}
&\cite{neveux_completed_2020}
&\cite{blake_wigglez_2012}
&\cite{blake_wigglez_2012}
&\cite{blake_wigglez_2012} \\

\hline\hline
\end{tabular}

\end{table}


==> 2nd_V_Testing_Large-Scale Structure_Measurements_Against_Fisher_Matrix_Predictions/table3.tex <==

\begin{table}[t]
\centering
\caption{\label{tab:results2} Same as Table \ref{tab:results}, but including intermediate data releases of BOSS and eBOSS. LOWZ and CMASS are shortened as LZ and CM. \\}
\begin{tabular}{||c||c|c c|c c|c c|c c|c c||}
\hline\hline
  & BOSS & \multicolumn{2}{c|}{BOSS DR10} & \multicolumn{2}{c|}{BOSS DR11} &
  \multicolumn{2}{c|}{BOSS DR12} &
  \multicolumn{2}{c|}{eBOSS DR14} &
  \multicolumn{2}{c||}{eBOSS DR16}
  \\

  & DR9
  & LZ & CM 
  & LZ & CM 
  & LZ & CM 
  & $\rm LRG^{+}$  & QSO
  & $\rm LRG^{+}$  & QSO
  \\
  
\hline
$z_{\rm eff}$&
0.57&	0.32&	0.57& 	0.32&	0.57& 0.32&	0.57&	0.72&	1.52&  0.698&  1.48\\

$A_{\rm eff}(deg^2)$ & 
3275&	5156&	6161&	7341&	8377&  8337&	9376&	1845&	2113&  9494&   4699\\

$V_{eff}(Gpc^3)$&

2.474&	1.770&	4.669&	2.527&	6.381&  2.185&	5.034&	0.910&	0.218&  2.652&  0.525\\

$b_{\rm eff}$& 
2.0&  1.8&  2.11& 1.85&  2.05&   1.9&   2.1&   2.0&  2.63 & 2.2& 2.33\\

\hline\hline
\multicolumn{12}{c}{Fractional errors from the BAO analysis (in percent)}\\
\hline\hline

$D_M$(O.)&
2.0&	&	1.9&	&	1.4&  2.2&   1.3&	 &	 &  1.6&   2.5  \\

$D_M$(F.)&
2.2&	2.7&	1.6&	2.2&	1.4&	2.0&	1.3&	3.2&	5.2&    1.7&    3.4\\ 
\hline

$D_H$(O.)&
3.8&	&	5.0&	&	3.5& 5.9& 2.9&	&	 & 2.5&   4.0\\

$D_H$(F.)&
4.4&	5.4&	3.1&	4.5&	2.7&	4.2&	2.5&	5.9&	7.8&    3.2&    5.0\\
\hline

$D_V$(O.)&
1.6&	2.8&	1.4&	2.0&	0.9&  1.7&  0.9&  2.5&	3.8& 1.6&  1.5\\

$D_V$(F.)&
1.6&	2.0&	1.1&	1.6&	1.0&	1.5&	0.9&	2.2&	3.9&    1.2&    3.0\\
\hline

BAO ref. 
& \cite{anderson_clustering_2012} 
&\cite{anderson_clustering_2014}
&\cite{anderson_clustering_2014}
&\cite{anderson_clustering_2014}
&\cite{anderson_clustering_2014}
&\cite{gil-marin_clustering_2016-2}
&\cite{gil-marin_clustering_2016-2}
&\cite{bautista_sdss-iv_2018}
&\cite{ata_clustering_2018}
&\cite{bautista_completed_2020}
&\cite{neveux_completed_2020}\\

\hline\hline
\multicolumn{12}{c}{Fractional errors from the RSD analysis (in percent)}\\
\hline\hline

$f \sigma_8$(O.Mg.)&
%The fs used to 0.127 be from this paper: https://arxiv.org/pdf/1310.1106.pdf

14.6&   23.3&   12.8&   20.8&	9.9&   15.7&   8.6&	29.2&	16.4& 7.9& 9.3\\

$f \sigma_8$(O.Fx.)&
8.1&       &	    &      &	6.0&	9.1&   5.0&    10.4&	15.4& 7.6&  6.3\\

$f \sigma_8$(F.Fx.)&
4.5&	6.2&	3.3&	5.3&	2.8&	5.0&	2.7&	5.2&	5.9&    3.1&    4.0\\

\hline\hline
\multicolumn{12}{c}{$k_{max}$ for the RSD modeling}\\
\hline\hline

$k_{\rm max}$(O.)&
0.14& 0.09& 0.09& 0.09& 0.14&
0.17&	0.17&	0.13&	0.18&	0.16&	0.24\\

$k_{\rm max}$(Fid. F.)&
0.13&	0.12&	0.13&	0.12&	0.13&	0.12&	0.13&	0.15&	0.20&  0.14&  0.20\\
$k_{\rm max}$(Match)&
0.08&	&	&	&	0.07&	0.08&	0.08&	0.08&	0.07&  0.07& 0.08\\

\hline
RSD Model&
R+11
& & &
& R+11 %\cite{reid_towards_2011}
&
\multicolumn{2}{c|}{TNS}&
\multicolumn{2}{c|}{CLPT+GS}&
\multicolumn{2}{c||}{TNS\&CLPT}\\

 RSD space&
 $s$ &
 $s$ &
 $s$ &
 $s$ &
 $s$ &
 $k$ &
 $k$ &
 $s$ &
 $s$ &
 $s$ &
 $k$/$s$ \\

RSD ref. 
& \cite{reid_clustering_2012}
& \cite{sanchez_clustering_2014}
& \cite{sanchez_clustering_2014}
& \cite{sanchez_clustering_2014}
&\cite{samushia_clustering_2014}
&\cite{gil-marin_clustering_2016}
&\cite{gil-marin_clustering_2016}
&\cite{icaza-lizaola_clustering_2020}
&\cite{zarrouk_clustering_2018} &\cite{bautista_completed_2020}
&\cite{neveux_completed_2020}\\

\hline\hline

\end{tabular}
\end{table}

==> 2nd_V_Testing_Large-Scale Structure_Measurements_Against_Fisher_Matrix_Predictions/table4.tex <==

\begin{table}[h]
\centering
\caption{\label{tab:results3} The fractional error of $f \sigma_8^{\rm mg.\alpha s}$ in percent and the $k_{\rm max}$ at which observed (O.) and Fisher (F.) errors match. In contrast to Table \ref{tab:results}, the Fisher prediction errors are calculated after marginalizing over the dilation parameters (Mg.).}
\begin{tabular}{||c||c|c|cc|ccc|ccc||}
\hline\hline
  & 6dFGS
  & MGS 
  & \multicolumn{2}{c|}{BOSS} 
  & \multicolumn{3}{c|}{eBOSS} & \multicolumn{3}{c||}{WiggleZ}\\
  &
  & 
  & Near  &  Mid
  & $\rm LRG^{+}$ & ELG & QSO 
  & Near&	Mid&	Far
  \\
\hline

$f \sigma_8$(O.Mg.)&
-&  40.5&	7.8&	7.6&	7.9&
23.6&	9.3&	19.4&	16.1&	16.4	\\

$f \sigma_8$(F.Mg.)&

 -&   30.1&	7.8&	6.7&	6.5&	7.9&	7.3&	11.5&	9.5&	11.4	\\

\hline

$k_{\rm max}$(Match)&

-&   0.084&	0.122&	0.117&	0.113&	0.060&	0.104&	0.083&	0.086&	0.094\\

\hline\hline
 
\end{tabular}

\end{table}

==> 2nd_V_Testing_Large-Scale Structure_Measurements_Against_Fisher_Matrix_Predictions/table5.tex <==

\begin{table}[h]
\centering

\caption{\label{tab:results4} Same as Table \ref{tab:results3} but including intermediate data releases.}
\begin{tabular}{||c||c|cc|cc|cc|cc|cc||}
\hline\hline
  & BOSS & \multicolumn{2}{l|}{BOSS DR10} & \multicolumn{2}{c|}{BOSS DR11} &
  \multicolumn{2}{c|}{BOSS DR12} &
  \multicolumn{2}{c|}{eBOSS DR14} &
  \multicolumn{2}{c||}{eBOSS DR16}
  \\

  & DR9
  & LZ & CM 
  & LZ & CM 
  & LZ & CM 
  & $\rm LRG^{+}$  & QSO
  & $\rm LRG^{+}$  & QSO
  \\
  
\hline

$f \sigma_8$(O.Mg.)&
%The fs used to 0.127 be from this paper: https://arxiv.org/pdf/1310.1106.pdf

14.6&   23.3&   12.8&   20.8&	9.9&   15.7&   8.6&	29.2&	16.4& 7.9& 9.3\\

$f \sigma_8$(F.Mg.)&

9.2&	12.9&	7.0&	11.1&	5.9&	10.6&	5.7&	10.5&	10.9&   6.5&    7.3\\

\hline

$k_{\rm max}$(Match)&
0.087&	0.073&	0.081&	0.072&	0.085&	0.082&	0.090&	0.054&	0.093& 0.113&	0.104 \\

\hline\hline
\end{tabular}
\end{table}
